Bridging Language and Action: A Survey of Language-Conditioned Robot Manipulation

Language-conditioned robot manipulation is an emerging field aimed at enabling seamless communication and cooperation between humans and robotic agents by teaching robots to comprehend and execute instructions conveyed in natural language. This interdisciplinary area integrates scene understanding, language processing, and policy learning to bridge the gap between human instructions and robot actions. In this comprehensive survey, we systematically explore recent advancements in language-conditioned robot manipulation. We categorize existing methods based on the primary ways language is integrated into the robot system, namely language for state evaluation, language as a policy condition, language for cognitive planning and reasoning, and language in unified vision-language-action models. Specifically, we further analyze state-of-the-art techniques from five axes of action granularity, data and supervision regimes, system cost and latency, environments and evaluations, and task specification. Additionally, we highlight the key debates in the field. Finally, we discuss open challenges and future research directions, focusing on potentially enhancing generalization capabilities and addressing safety issues in language-conditioned robot manipulators.

==> sections/approaches-code-new-with-code.tex <==

\begin{table*}[htbp]
    \centering
    \caption{\textcolor{black}{Comparison of language-condition robot manipulation approaches II}}
    \begin{threeparttable}
    \begin{adjustbox}{width=\linewidth,center}
        \begin{tabular}{ l c c c c c c c c c c}
            \toprule
            Models & Years & \makecell{Benchmark or\\ \textit{Simulation Engine}} & \makecell{Language \\ Module} & \makecell{Perception \\ Module} & \makecell{Real world \\experiments} & FMs & \makecell{RL} & \makecell {IL} & \makecell {MP} & {Released Code}\\
            
              \midrule
              Ground4Act~\citeauthor{YANG2024105280} & 2024 & Gazebo & Transformer & ResNet101, BERT & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark}  & \textcolor{JungleGreen}{\cmark}\\
              LOVM~\citeauthor{ye2024task} & 2024 & \# & BiGRU & LOVM & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} &  \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark}  & \textcolor{Salmon}{\xmark}\\
              ECLAIR~\citeauthor{10803055} & 2024 & \# & GPT-3-turbo & * & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark}\\
              PR2L~\citeauthor{chen2024visionlanguagemodelsprovidepromptable} & 2024 & MineDojo, HM3D & InstructBLIP & InstructBLIP & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}  & \textcolor{Salmon}{\xmark}  & \textcolor{JungleGreen}{\cmark}\\
              AHA~\citeauthor{duan2024ahavisionlanguagemodeldetectingreasoning} & 2024 & RLBench, ManiSkill, RoboFail & LLaMA-2-13B & CLIP & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\
              KOI~\citeauthor{lu2024koiacceleratingonlineimitation} & 2024 & Meta-World, LIBERO & GPT-4v & KOI & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\
              GPT-4V(ISION)~\citeauthor{10711245} & 2024 & \# & GPT-4 & GPT-4 & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark}\\
              HiRT~\citeauthor{zhang2025hirtenhancingroboticcontrol} & 2024 & Meta-World, Franka-Kitchen & InstructBLIP & CNN & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark}\\
              Sentinel~\citeauthor{agia2024unpackingfailuremodesgenerative} & 2024 & \# & GPT-4o & PointNet++ & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\
              
              RoLD~\citeauthor{tan2024roldrobotlatentdiffusion} & 2024 & Open X-E, Robomimic, Meta-World & DistilBERT & DistilBERT & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              
              \midrule
              
              ITS~\citeauthor{Jin2025} & 2025 & * & LLaMA & A2C & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\
              SIAMS~\citeauthor{hatanaka2025reinforcement} & 2025 & Miniworld & LTL & CNN & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} &  \textcolor{JungleGreen}{\cmark}\\
              CRTO~\citeauthor{10955186} & 2025 & Continual World & ChatGPT & * & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              LAMARL~\citeauthor{ZhuLAMARL} & 2025 & \textcolor{Salmon}{\xmark} & OpenAI & MADDPG & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\
              ARCHIE~\citeauthor{TurcatoARCHIE} & 2025 & \# & GPT-4 & * & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\
              RealBEF~\citeauthor{wang2025guiding} & 2025 & Meta-World & ALBEF & CNN & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark}\\
              LLMRewardShaping~\citeauthor{guo2024utilizing} & 2025 & Meta-World & GPT-4 & * & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark}\\
              BOSS~\citeauthor{YangBOSS} & 2025 & LIBERO & OpenVLA & ResNet & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\
              LAV-ACT~\citeauthor{TripathiLAV-ACT} & 2025 & MuJuCo & Voltron & Voltron & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark}\\
              TPM~\citeauthor{YangTPM} & 2025 & MuJuCo & GPT-4 & ResNet & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\
              Mamba~\citeauthor{10966860} & 2025 & \# & Mamba & Mamba & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              TransformerPolicy~\citeauthor{10934975} & 2025 & CALVIN & Transformer & Sentence-BERT & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              HierarchicalLCL~\citeauthor{10.1007/978-981-96-1614-5_11} & 2025 & CALVIN & OpenFlamingoM-3B & ViT & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              BLADE~\citeauthor{liu2024learning} & 2025 & CALVIN & GPT-4 & PCT & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              LES6DPose~\citeauthor{11075556} & 2025 & Isaac Gym & GPT-4 & PointNet++ & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              SafetyFilter~\citeauthor{10933541} & 2025 & \# & GPT-4o & CLIP & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              TARAD~\citeauthor{11124589} & 2025 & RLBench & GPT-4o & CLIP & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              DISCO~\citeauthor{hao2025language} & 2025 & CALVIN & GPT-4o & * & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              TinyVLA~\citeauthor{10900471} & 2025 & Meta-World & Pythia & MLP & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\
              ASD-QR~\citeauthor{wang2025integrating} & 2025 & ScalingUp & GPT3 & CLIP & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              RDT-1B~\citeauthor{liu2025rdt1bdiffusionfoundationmodel} & 2025 & \# & GPT-4-Turbo & T5-XXL & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark}\\
              GRAVMAD~\citeauthor{chen2025gravmad} & 2025 & RLBench & GPT-4o & CLIP & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\
              GR-MG~\citeauthor{li2025gr} & 2025 & CALVIN & Transformer & T5-Base & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark}\\  LEMMo-Plan~\citeauthor{chen2025lemmo} & 2025 & \textcolor{Salmon}{\xmark} & GPT-4o & * & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}\\              
            \bottomrule
        \end{tabular}
        \end{adjustbox}
        \begin{tablenotes}
        \small \# their own benchmark; * directly get environment states; FMs: use foundational models or not; \\
        \small RL: Reinforcement Learning; IL: Imitation Learning; MP: Motion Planning;
        \end{tablenotes}
    \end{threeparttable}
    
    \label{tab:approaches-v2}
\end{table*}

==> sections/approaches-vla-table-all-v2.tex <==
\begin{table*}[t]
\centering
\caption{\textcolor{black}{Classification of VLA models and design dimensions}}
\begin{threeparttable}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ l l c c c c c c c c c c c c c c c c c c }
\toprule
\multicolumn{1}{c}{Optimization} & \multicolumn{1}{c}{Article} & \multicolumn{2}{c}{Observation} & \multicolumn{4}{c}{Action generation} & \multicolumn{4}{c}{VLM policy} & \multicolumn{4}{c}{Pretraining} & \multicolumn{3}{c}{Scenarios} \\
 \cmidrule(lr){2-2} \cmidrule(lr){3-4} \cmidrule(lr){5-8} \cmidrule(lr){9-12} \cmidrule(lr){13-16} \cmidrule(lr){17-19}
\multicolumn{1}{c}{Direction} &  &  &  &  &  &  &  & CoT & FP & MEM & OP & MD & CE & HD & AF & MS & RW & CE \\

\midrule
 
Spatial & SpatialVLA\cite{qu2025spatialvla} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Autoregressive} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
Understanding & BridgeVLA\cite{li2025bridgevla} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{DirectPred} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & PointVLA\cite{li2025pointvla} & \multicolumn{2}{c}{RGBD, ROB, TX} & \multicolumn{4}{c}{Diffusion Model} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & GeoVLA\cite{sun2025geovla} & \multicolumn{2}{c}{RGBD, ROB, TX} & \multicolumn{4}{c}{Diffusion Model} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
\midrule
 
Data Source \& & EgoVLA\cite{yang2025egovla} &\multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{DirectPred} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\
Augmentation & H-RDT\cite{bi2025h} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Flow Matching} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & Shortcut\cite{xing2025shortcut} & \multicolumn{2}{c}{RGB, TX} & \multicolumn{4}{c}{Not Applicable} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 
\midrule
 
Multimodal & ForceVLA\cite{yu2025forcevla} & \multicolumn{2}{c}{RGBD, ROB, TX} & \multicolumn{4}{c}{Flow Matching} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
Sensing \& & Tactile-VLA\cite{huang2025tactile} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Flow Matching} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
Fusion & VTLA\cite{zhang2025vtla} & \multicolumn{2}{c}{RGB, TX} & \multicolumn{4}{c}{Autoregressive} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & OmniVTLA\cite{cheng2025omnivtla} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Flow Matching} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\

 \midrule
 
Reasoning \& & CoT-VLA\cite{zhao2025cot} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Autoregressive} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
World Models & Seer\cite{tian2025predictive} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{DirectPred} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
& WorldVLA\cite{cen2025worldvla} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Autoregressive} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
& DreamVLA\cite{zhang2025dreamvla} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Diffusion Model} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Knowledge & ChatVLA\cite{zhou2025chatvla} &\multicolumn{2}{c}{RGB, TX} &  \multicolumn{4}{c}{Diffusion Model} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
Preserving & ChatVLA-2\cite{zhou2025vision} & \multicolumn{2}{c}{RGB, TX} &  \multicolumn{4}{c}{Diffusion Model} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}  & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & Insulating\cite{driess2025knowledge} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{FM + AR} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & DiffusionVLA\cite{wen2025diffusionvla} & \multicolumn{2}{c}{RGBD, TX} & \multicolumn{4}{c}{DM + AR} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & InstructVLA\cite{yang2025instructvla} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Flow Matching} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & GR-3\cite{cheang2025gr} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Flow Matching} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\


 
\midrule
 
Long-horizon & Long-VLA\cite{fan2025long} & \multicolumn{2}{c}{RGB, TX} & \multicolumn{4}{c}{Diffusion Model} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
task solving & DexVLA\cite{wen2025dexvla} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Diffusion Model} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
& MemoryVLA\cite{shi2025memoryvla} & \multicolumn{2}{c}{RGB, TX} & \multicolumn{4}{c}{Diffusion Model} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
& LoHoVLA\cite{yang2025lohovla} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Autoregressive} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
Policy & PI-0\cite{black2024pi_0} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Flow Matching} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
Execution & PI-Fast\cite{pertsch2025fast} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Flow Matching} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
& PI-0.5\cite{pmlr-v305-black25a} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Flow Matching} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\

 \midrule
 
Adaptation \& & OpenVLA-OFT\cite{kim2025fine} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{DirectPred} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
Fine-Tuning & ControlVLA\cite{li2025controlvla} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Diffusion Model} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
& ConRFT\cite{chen2025conrft} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Diffusion Model} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
& RIPT-VLA\cite{tan2025interactive} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Autoregressive} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
& DisDiffVLA\cite{liang2025discrete} & \multicolumn{2}{c}{RGB, ROB, TX} & \multicolumn{4}{c}{Diffusion Model} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\

\bottomrule
\end{tabular}}
    \begin{tablenotes}
        \small Observation: RGB images, D: depth information (e.g., point clouds), ROB: Robot Proprioception, TX: text (e.g., prompt, language goal). \\
        \small Action generation: FM-Flow Matching, DM-Diffusion Model, AR-Autoregressive, DP-Direct Prediction;
    \end{tablenotes}
\end{threeparttable}
\label{tab:vla_table}
\end{table*}


==> sections/approaches-vla-table-all.tex <==
\begin{table*}[t]
\centering
\caption{\textcolor{black}{Classification of VLA models and design dimensions}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ l l c c c c c c c c c c c c c c c c c c c c }
\toprule
\multicolumn{1}{c}{Direction} & \multicolumn{1}{c}{Article} & \multicolumn{4}{c}{Observation} & \multicolumn{4}{c}{Action generation} & \multicolumn{4}{c}{VLM policy} & \multicolumn{4}{c}{Pretraining} & \multicolumn{3}{c}{Scenarios} \\
 \cmidrule(lr){2-2} \cmidrule(lr){3-6} \cmidrule(lr){7-10} \cmidrule(lr){11-14} \cmidrule(lr){15-18} \cmidrule(lr){19-21}
 &  & RGB & DH & PN & TX & DM & FM & AR & DP & CoT & FP & MEM & OP & MD & CE & HD & AF & MS & RW & CE \\
\midrule
Action & PI-0\cite{black2024pi_0} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 Optimization & PI-Fast\cite{pertsch2025fast} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & PI-0.5\cite{pmlr-v305-black25a} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\

 \midrule
 
Fine-tuning & openVLA-OFT\cite{kim2025fine} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & ControlVLA\cite{li2025controlvla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & ConRFT\cite{chen2025conrft} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & RIPT-VLA\cite{tan2025interactive} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Discrete diffusion VLA\cite{liang2025discrete} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\

\midrule
 
Future state & CoT-VLA\cite{zhao2025cot} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 Prediction & Seer\cite{tian2025predictive} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & WorldVLA\cite{cen2025worldvla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & DreamVLA\cite{zhang2025dreamvla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Spatial & SpatialVLA\cite{qu2025spatialvla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
Understanding & BridgeVLA\cite{li2025bridgevla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & PointVLA\cite{li2025pointvla} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & GeoVLA\cite{sun2025geovla} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Knowledge & ChatVLA\cite{zhou2025chatvla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} &  \textcolor{JungleGreen}{\cmark} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
Preserving & ChatVLA-2\cite{zhou2025vision} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} &  \textcolor{JungleGreen}{\cmark} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark}  & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & Knowledge Insulating\cite{driess2025knowledge} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} &  \textcolor{JungleGreen}{\cmark} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} &  \textcolor{JungleGreen}{\cmark} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & DiffusionVLA\cite{wen2025diffusionvla} & \textcolor{JungleGreen}{\cmark} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} &  \textcolor{JungleGreen}{\cmark} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} &  \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & InstructVLA\cite{yang2025instructvla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & GR-3\cite{cheang2025gr} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Training Data & EgoVLA\cite{yang2025egovla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\
 & H-RDT\cite{bi2025h} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & Shortcut learning\cite{xing2025shortcut} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Long Horizon & Long-VLA\cite{fan2025long} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & DexVLA\cite{wen2025dexvla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & MemoryVLA\cite{shi2025memoryvla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & LoHoVLA\cite{yang2025lohovla} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Multi-modal & ForceVLA\cite{yu2025forcevla} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
Perception & Tactile-VLA\cite{huang2025tactile} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & VTLA\cite{zhang2025vtla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & OmniVTLA\cite{cheng2025omnivtla} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
\bottomrule
\end{tabular}}
\label{tab:vla_table}
\end{table*}


==> sections/approaches-vla-table-clean.tex <==

\begin{table*}[t]
\centering
\caption{\textcolor{black}{Classification of VLA models and design dimensions} \textcolor{red}{Is it multi-model perception or multi-modal perception????}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ l l c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c }
\toprule
\multicolumn{1}{c}{optimization direction} & \multicolumn{1}{c}{Article} & \multicolumn{5}{c}{Input} & \multicolumn{6}{c}{Control strategy: action generation} & \multicolumn{4}{c}{VLM policy} & \multicolumn{6}{c}{Pretraining} & \multicolumn{2}{c}{RL} & \multicolumn{5}{c}{Purpose: scenarios} & \multicolumn{5}{c}{Purpose: challenges} \\
 \cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-13} \cmidrule(lr){14-17} \cmidrule(lr){18-23} \cmidrule(lr){24-25} \cmidrule(lr){26-30} \cmidrule(lr){31-35}
 & Article & RGB & DH & PN & OS & TX & DM & FM & GM & NR & AR & NC & CoT & FP & MEM & OP & ID & OD & CE & VD & HD & AF & AF & ACT & ST & SS & MS & RW & CE & CL & GL & DE & TE & IE \\
\midrule
Action & PI-0\cite{black2024pi_0} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\
 & PI-Fast\cite{pertsch2025fast} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & PI-0.5\cite{intelligence2025pi_05} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\
 & Real-time chunking & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

 \midrule
 
Efficient fine-tuning & openVLA-OFT & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & ControlVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & ConRFT & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & RIPT-VLA & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Discrete diffusion VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Future state prediction & CoT-VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Seer & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & WorldVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & DreamVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Spatial Understanding & SpatialVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & BridgeVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & PointVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & GenVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Knowledge Preserving & ChatVLA & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & ChatVLA-2 & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Knowledge Insulating VLA & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & DiffusionVLA & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & InstructVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\
 & GR-3 & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\

\midrule
 
Training Data & EgoVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & H-RDT & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Shortcut learning in VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & CAST & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Long Horizon & Long-VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & DexVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & MemoryVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & LoHoVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Multi-modal Perception & ForceVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Tactile-VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & VTLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & OmniVTLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
\bottomrule
\end{tabular}}
\label{tab:vla_table}
\end{table*}

==> sections/approaches-vla-table.tex <==

\begin{table*}[t]
\centering
\caption{\textcolor{black}{Classification of VLA models and design dimensions} \textcolor{red}{Is it multi-model perception or multi-modal perception????}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ l l c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c c }
\toprule
\multicolumn{1}{c}{optimization direction} & \multicolumn{1}{c}{Article} & \multicolumn{5}{c}{Input} & \multicolumn{6}{c}{Control strategy: action generation} & \multicolumn{5}{c}{Control strategy: task planner} & \multicolumn{4}{c}{VLM policy} & \multicolumn{6}{c}{Pretraining} & \multicolumn{2}{c}{RL} & \multicolumn{5}{c}{Purpose: scenarios} & \multicolumn{5}{c}{Purpose: challenges} \\
 \cmidrule(lr){2-2} \cmidrule(lr){3-7} \cmidrule(lr){8-13} \cmidrule(lr){14-18} \cmidrule(lr){19-22} \cmidrule(lr){23-28} \cmidrule(lr){29-30} \cmidrule(lr){31-35} \cmidrule(lr){36-40}
 & Article & RGB & DH & PN & OS & TX & DM & FM & GM & NR & AR & NC & DM & FM & NR & NC & AF & CoT & FP & MEM & OP & ID & OD & CE & VD & HD & AF & AF & ACT & ST & SS & MS & RW & CE & CL & GL & DE & TE & IE \\
\midrule
Action & PI-0 & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\
 & PI-Fast & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} \\
 & PI-0.5 & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\
 & Real-time chunking & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

 \midrule
 
Efficient fine-tuning & openVLA-OFT & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & ControlVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & ConRFT & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & RIPT-VLA & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Discrete diffusion VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Future state prediction & CoT-VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Seer & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & WorldVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & DreamVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Spatial Understanding & SpatialVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & BridgeVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & PointVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & GenVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Knowledge Preserving & ChatVLA & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & ChatVLA-2 & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Knowledge Insulating VLA & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & DiffusionVLA & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & InstructVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\
 & GR-3 & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} \\

\midrule
 
Training Data & EgoVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & H-RDT & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Shortcut learning in VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & CAST & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Long Horizon & Long-VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & DexVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} \\
 & MemoryVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & LoHoVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\

\midrule
 
Multi-modal Perception & ForceVLA & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & Tactile-VLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & VTLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
 & OmniVTLA & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{JungleGreen}{\cmark} & \textcolor{Salmon}{\xmark} & \textcolor{Salmon}{\xmark} \\
\bottomrule
\end{tabular}}
\label{tab:vla_table}
\end{table*}
